Effects of Pycnonuclear Reactions on White Dwarf Stellar Evolution

This document presents a numerical study of the effects of high density nuclear reactions, pycnonuclear reactions, on the evolution of white dwarfs that accrete matter from a companion star. Primarily we seek observable properties that might be different when we include these nuclear reactions with varying microphysical assumptions. These different assumptions include effective nucleon-nucleon interactions, lattice structures and crystal polarization characteristics. Our results indicate that, although we find some significant differences in pycnonuclear reaction rates, the differences do not result in observable differences in the white dwarf evolution. Secondarily we examine the differences in observable properties when pycnonuclear reactions are assumed to happen and when they are assumed to not happen. In this case, our calculations indicate there can be observable differences in the radius, $R$, and the effective temperature, $T_{eff}$, at the stopping condition we use for our simulations, $L_{nuc} > 10^{8}\thinspace \rm{L}_{\odot}$, that is the total rate of energy released by nuclear fusion is greater than $10^{8}$ solar luminosities. Thirdly we explore the often neglected effect of temperature enhancement to pycnonuclear rates.

==> Makefile <==
PS2PDF_OPTS=-dEmbedAllFonts=true -dPDFSETTINGS=/prepress

all: thesis.pdf

datestamp:
	rm -f ../THIS-IS-VERSION*
	touch ../THIS-IS-VERSION-`date +%F-%T`

view: thesis.ps
	gv thesis.ps

thesis.dvi: *.bib Figures/*.eps *.tex *.cls
	( latex thesis || rm -f thesis.dvi ) && \
	makeglossaries thesis && \
	bibtex thesis && \
	( latex thesis || rm -f thesis.dvi ) && \
	( latex thesis || rm -f thesis.dvi ) && \
	( latex thesis || rm -f thesis.dvi )

thesis.ps: thesis.dvi
	dvips -t letter -o thesis.ps thesis

thesis.pdf: thesis.ps
	ps2pdf ${PS2PDF_OPTS} thesis.ps thesis.pdf

clean:
	rm -vf *.aux *.bbl *.blg *.dvi *.ps *.pdf *.log *.lot *.toc \
	*.lof *.gls *.glg *.ist *.glo *~ ../.DS_Store .DS_Store
	rm -rf ../data_analysis/.ipynb_checkpoints/

